Classifying the full SDSS-IV MaNGA Survey using optical diagnostic diagrams: presentation of AGN catalogs in flexible apertures

Accurate active galactic nucleus (AGN) identifications in large galaxy samples are crucial to assess the role of AGN and AGN feedback in the coevolution of galaxies and their central supermassive black holes. Emission line flux ratio diagnostics are the most common technique for identifying AGN in optical spectra. New large samples of integral field unit observations allow The exploration of the role of aperture size used for the classification. In this paper, we present galaxy classifications for all 10,010 galaxies observed within the Mapping Nearby Galaxies at Apache Point Observatory (MaNGA) survey. We use Baldwin-Philips-Terlevich line flux ratio diagnostics combined with an H$\alpha$ equivalent threshold in 60 apertures of varying size for the classification and provide the corresponding catalogs. MaNGA-selected AGN primarily lie below the main sequence of star-forming galaxies, reside with massive galaxies with stellar masses of $\sim 10^{11}$~M$_{\odot}$ and a median H$\alpha$-derived star formation rate of $\sim 1.44$M$_{\odot}$~yr$^{-1}$. We find that the number of `fake' AGN increases significantly beyond selection apertures of $>$~1.0~R$_{eff}$ due to increased contamination from diffuse ionized gas (DIG). A comparison with previous works shows that the treatment of the underlying stellar continuum and flux measurements can significantly impact galaxy classification. Our work provides the community with AGN catalogs and galaxy classifications for the full MaNGA.

==> a_try.tex <==
\section{nothing}
